A rigorous introduction to linear models

This book is meant to provide an introduction to linear models and the theories behind them. Our goal is to give a rigorous introduction to the readers with prior exposure to ordinary least squares. In machine learning, the output is usually a nonlinear function of the input. Deep learning even aims to find a nonlinear dependence with many layers, which require a large amount of computation. However, most of these algorithms build upon simple linear models. We then describe linear models from different perspectives and find the properties and theories behind the models. The linear model is the main technique in regression problems, and the primary tool for it is the least squares approximation, which minimizes a sum of squared errors. This is a natural choice when we're interested in finding the regression function which minimizes the corresponding expected squared error. This book is primarily a summary of purpose, significance of important theories behind linear models, e.g., distribution theory and the minimum variance estimator. We first describe ordinary least squares from three different points of view, upon which we disturb the model with random noise and Gaussian noise. Through Gaussian noise, the model gives rise to the likelihood so that we introduce a maximum likelihood estimator. It also develops some distribution theories via this Gaussian disturbance. The distribution theory of least squares will help us answer various questions and introduce related applications. We then prove least squares is the best unbiased linear model in the sense of mean squared error, and most importantly, it actually approaches the theoretical limit. We end up with linear models with the Bayesian approach and beyond.

==> end.tex <==
\backmatter
\clearpage

\pagestyle{empty}
\begin{center}
	\bfseries
\vspace{1cm}
	\Huge
	{\huge
		{Publisher: Eliva Press Global Ltd}}
	
{\huge
	{Email: info@elivapress.com}}
	
\vspace{1cm}
	\normalsize
	

\vspace{1cm}
%	\small BY\\
	
\vspace{1cm}
\vspace{1cm}
	\normalsize
	
\vspace{1cm}
	\large
All rights reserved
\end{center}



\clearpage
\pagestyle{empty}
\begin{flushleft}
	\large
\textbf{Eliva Press} is an independent international publishing house established for the publication and dissemination of academic works all over the world. Company provides high quality and professional service for all of our authors.


\vspace{1cm}

Our Services:
Free of charge, open-minded, eco-friendly, innovational.

\vspace{1cm}

- Free standard publishing services (manuscript review, step-by-step book preparation, publication, distribution, and marketing).

- No financial risk. The author is not obliged to pay any hidden fees for publication.

- Editors. Dedicated editors will assist step by step through the projects. 

- Money paid to the author for every book sold. Up to 50\% royalties guaranteed. 

- ISBN (International Standard Book Number). We assign a unique ISBN to every Eliva Press book.

- Digital archive storage. Books will be available online for a long time. We don't need to have a stock of our titles. No unsold copies. Eliva Press uses environment friendly print on demand technology that limits the needs of publishing business. We care about environment and share these principles with our customers. 

- Cover design. Cover art is designed by a professional designer. 

- Worldwide distribution. We continue expanding our distribution channels to make sure that all readers have access to our books.



\bfseries
\vspace{1cm}
%\Huge
%{\nbtitlestretch\Huge
%\mytitle}

\vspace{1cm}
\normalsize

\vspace{4cm}

\vspace{1cm}

\normalsize


\huge
\bfseries
\gap\gap\qquad www.elivapress.com
\vspace{1cm}
\end{flushleft}



==> front.tex <==
%\frontmatter
\begingroup
\clearpage

\pagestyle{empty}
\begin{center}
	\bfseries
\vspace{1cm}
	\Huge
	{\Huge
		{\mytitle}}
	
\vspace{1cm}
	\normalsize
	

\vspace{1cm}
%	\small BY\\
	
\vspace{1cm}
	
\vspace{1cm}
	\normalsize
	
\vspace{1cm}
\end{center}

\clearpage
\newpage\null\thispagestyle{empty}\newpage

\clearpage
\pagestyle{empty}
\begin{center}
	\bfseries
\vspace{1cm}
	\Huge
	{\Huge
		\mytitle}
	
	\vspace{1cm}
	\normalsize
	
%	TO WHICH IS ADDED MANY USEFUL ONE\\
%	LINERS AND CODE SO THAT\\
%	YOU CAN AWK LIKE A HAWK
\vspace{1cm}
	\small BY\\
	\Large Jun Lu\\[0.5em]
%	\footnotesize AUTHOR OF ``A WOINRKG ALGEBRA,'' ``STATISTICS,\\
%	ITS HISTORY, THEORY AND PRACTICE,'' ETC., ETC.
	
\vspace{1cm}
	
	%	\includegraphics[width=1.5in]{./graphics/pic37}
\vspace{1cm}
	\normalsize
	
\vspace{10cm}

\large
\gap\gap\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad  \gap ELIVA PRESS
\vspace{1cm}
\end{center}



\clearpage
\pagestyle{empty}
\begin{flushleft}
\bfseries
ISBN: 978-99949-8-189-2

\copyright
\bfseries
 Eliva Press Global Ltd. part of Eliva Press S.R.L., 2022

\copyright
\bfseries
 Jun Lu

Cover Design: Eliva Press

Cover Image: Freepik Premium

Email: info@elivapress.com

Website: www.elivapress.com

\vspace{1cm}

This Eliva Press imprint is published by the registered company Eliva Press Global Ltd. part of Eliva Press S.R.L. Publishing Group

\vspace{1cm}
The registered company address is: Pope Hennessy Street Level 2, Hennessy Tower Port Louis, Mauritius

Eliva Press S.R.L. Publishing Group address is: Bulevardul Moscova 21, Chisinau, Moldova, Europe

\vspace{1cm}
No part of this book may be reproduced or utilized in any form or by any means, electronic or mechanical, including photocopying, recording, or by any information storage and retrieval system, without permission in writing from Eliva Press or the author. Any brand and product names mentioned in this book are subject to the trademark, brand, or patent protection and are trademarks of their respective owners. The use of brand names, trade names, product names, product descriptions, is in no way implies that such names may be regarded as unrestricted by trademark and brand protection laws and thus may be used by anyone. The opinions and views expressed are exclusively those of the authors/contributors and in no way the editors or publisher is responsible.


\bfseries
\vspace{1cm}
%\Huge
%{\nbtitlestretch\Huge
%\mytitle}

\vspace{1cm}
\normalsize

%	TO WHICH IS ADDED MANY USEFUL ONE\\
%	LINERS AND CODE SO THAT\\
%	YOU CAN AWK LIKE A HAWK
\vspace{1cm}
%\small BY\\
%\Large Jun Lu\\[0.5em]
%%	\footnotesize AUTHOR OF ``A WOINRKG ALGEBRA,'' ``STATISTICS,\\
%	ITS HISTORY, THEORY AND PRACTICE,'' ETC., ETC.

\vspace{1cm}

%	\includegraphics[width=1.5in]{./graphics/pic37}
\vspace{1cm}
\normalsize


\large
%All rights reserved.
\vspace{1cm}
\end{flushleft}
\endgroup


==> symbols_theorems.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% colors
\usepackage[noframe]{showframe}
\usepackage{framed}
\usepackage{lipsum}


\makeatletter
\newcommand{\paragrapharrow}{%
	\@startsection{paragraph}{4}{\z@}%
	{3.25ex \@plus1ex \@minus.2ex}%
	{-1em}%
	{\normalfont\normalsize\bfseries$\blacktriangleright$\ }}
\makeatother

% margins 
\newcommand{\roundcornertheorem}{0pt}
\newcommand{\linewidththeorem}{0.1pt}
\newcommand{\frametitlerulewidththeorem}{0.1pt}
\newcommand{\innerbottommargintheorem}{2pt}
\newcommand{\innerleftmargintheorem}{2pt}
\newcommand{\innerrightmargintheorem}{2pt}
\newcommand{\innertopmargintheorem}{2pt}
\newcommand{\outerlinewidththeorem}{1pt}
\newcommand{\frametitleaboveskiptheorem}{1pt}

\newcommand{\textremark}{3pt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% new theorems
\renewcommand{\thesection}{\@arabic\c@section}
\newcounter{theo}[chapter] \setcounter{theo}{0}
%\renewcommand{\thetheo}{\arabic{section}.\arabic{theo}}
%\renewcommand{\thetheo}{\thechapter.\thesection.\arabic{theo}}
\renewcommand{\thetheo}{\thechapter.\arabic{theo}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Definition
%\newenvironment{definition}[1][]{%
	%	\refstepcounter{theo}%
	%	\ifstrempty{#1}%
	%	{\newcommand{\defName}{}}
	%	{\newcommand{\defName}{:~#1}}
	%	\mdfsetup{%
		%		frametitle={%
			%			\tikz[baseline=(current bounding box.east),outer sep=0pt]
			%			\node[anchor=east,rectangle,fill=\mdframecolorDefinition]
			%			{\strut Definition~\thetheo\defName};}}%
	%	\mdfsetup{innertopmargin=10pt,linecolor=\mdframecolorDefinition,%
		%		linewidth=2pt,topline=true,%
		%		frametitleaboveskip=\dimexpr-\ht\strutbox\relax
		%	}
	%	\begin{mdframed}[]\relax%
		%	}{\end{mdframed}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Remark
%\newenvironment{remark}[1][]{%
%	\refstepcounter{theo}%
%	\ifstrempty{#1}%
%	{\newcommand{\defName}{}}
%	{\newcommand{\defName}{:~#1}}
%	\mdfsetup{%
%		frametitle={%
%			\tikz[baseline=(current bounding box.east),outer sep=0pt]
%			\node[anchor=east,rectangle,fill=mdframecolorRemark]
%			{\strut Remark~\thetheo\defName};}}%
%	\mdfsetup{innertopmargin=10pt,linecolor=mdframecolorRemark,%
%		linewidth=2pt,topline=true,%
%		frametitleaboveskip=\dimexpr-\ht\strutbox\relax
%		% new added
%		frametitlerule=false, 
%		frametitlerulewidth=\frametitlerulewidththeorem,%    options when using {tcolorbox}?
%		%		roundcorner=\textremark,
%		%		linewidth=\textremark,
%		innertopmargin=\textremark,
%		innerbottommargin=\textremark,
%		innerleftmargin=\textremark,
%		innerrightmargin=\textremark,
%		frametitlebelowskip=3pt,
%		outerlinewidth=1.2pt,
%	}
%	\begin{mdframed}[]\relax%
%	}{\end{mdframed}}

%----------------------------------------------------------------------------------------
% Theorem Blues
%----------------------------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Theorem Blue
\newenvironment{theoremHigh}[1][]{%
\refstepcounter{theo}%
\ifstrempty{#1}%
{\newcommand{\theoName}{}}
{\newcommand{\theoName}{:~(#1)}}
\mdfsetup{
	backgroundcolor=structurecolorHighTheorem,
	linecolor=structurecolorHighTheorem,
	% ----------------------------------
	frametitlerulewidth=\frametitlerulewidththeorem,%    options when using {tcolorbox}?
	roundcorner=\roundcornertheorem,
	linewidth=\linewidththeorem,
	innerbottommargin=\innerbottommargintheorem,
	innerleftmargin=\innerleftmargintheorem,
	innerrightmargin=\innerrightmargintheorem,
	innertopmargin=\innertopmargintheorem,
	outerlinewidth=\outerlinewidththeorem,
	topline=false,
	innertopmargin=-5pt,
	innerbottommargin=1pt,
	linewidth=0,
	startinnercode=\paragraph{{\strut Theorem~\thetheo\theoName}}
}
\begin{mdframed}[]\relax%
}{\end{mdframed}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Corollary Blue
\newenvironment{corollaryHigh}[1][]{%
\refstepcounter{theo}%
\ifstrempty{#1}%
{\newcommand{\theoName}{}}
{\newcommand{\theoName}{:~(#1)}}
\mdfsetup{
	backgroundcolor=structurecolorHighTheorem,
	linecolor=structurecolorHighTheorem,
	% ----------------------------------
	frametitlerulewidth=\frametitlerulewidththeorem,%    options when using {tcolorbox}?
	roundcorner=\roundcornertheorem,
	linewidth=\linewidththeorem,
	innerbottommargin=\innerbottommargintheorem,
	innerleftmargin=\innerleftmargintheorem,
	innerrightmargin=\innerrightmargintheorem,
	innertopmargin=\innertopmargintheorem,
	outerlinewidth=\outerlinewidththeorem,
	topline=false,
	innertopmargin=-5pt,
	innerbottommargin=1pt,
	linewidth=0,
	startinnercode=\paragraph{{\strut Corollary~\thetheo\theoName}}
}
\begin{mdframed}[]\relax%
}{\end{mdframed}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Lemma Blue
\newenvironment{lemmaHigh}[1][]{%
\refstepcounter{theo}%
\ifstrempty{#1}%
{\newcommand{\theoName}{}}
{\newcommand{\theoName}{:~(#1)}}
\mdfsetup{
	backgroundcolor=structurecolorHighTheorem,
	linecolor=structurecolorHighTheorem,
	% ----------------------------------
	frametitlerulewidth=\frametitlerulewidththeorem,%    options when using {tcolorbox}?
	roundcorner=\roundcornertheorem,
	linewidth=\linewidththeorem,
	innerbottommargin=\innerbottommargintheorem,
	innerleftmargin=\innerleftmargintheorem,
	innerrightmargin=\innerrightmargintheorem,
	innertopmargin=\innertopmargintheorem,
	outerlinewidth=\outerlinewidththeorem,
	topline=false,
	innertopmargin=-5pt,
	innerbottommargin=1pt,
	linewidth=0,
	startinnercode=\paragraph{{\strut Lemma~\thetheo\theoName}}
}
\begin{mdframed}[]\relax%
}{\end{mdframed}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Proposition Blue
\newenvironment{propositionHigh}[1][]{%
\refstepcounter{theo}%
\ifstrempty{#1}%
{\newcommand{\theoName}{}}
{\newcommand{\theoName}{:~(#1)}}
\mdfsetup{
	backgroundcolor=structurecolorHighTheorem,
	linecolor=structurecolorHighTheorem,
	% ----------------------------------
	frametitlerulewidth=\frametitlerulewidththeorem,%    options when using {tcolorbox}?
	roundcorner=\roundcornertheorem,
	linewidth=\linewidththeorem,
	innerbottommargin=\innerbottommargintheorem,
	innerleftmargin=\innerleftmargintheorem,
	innerrightmargin=\innerrightmargintheorem,
	innertopmargin=\innertopmargintheorem,
	outerlinewidth=\outerlinewidththeorem,
	topline=false,
	innertopmargin=-5pt,
	innerbottommargin=1pt,
	linewidth=0,
	startinnercode=\paragraph{{\strut Proposition~\thetheo\theoName}}
}
\begin{mdframed}[]\relax%
}{\end{mdframed}}

%----------------------------------------------------------------------------------------
%   Theorem with grays
%----------------------------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Theorem
\newenvironment{theorem}[1][]{%
	\refstepcounter{theo}%
	\ifstrempty{#1}%
	{\newcommand{\theoName}{}}
	{\newcommand{\theoName}{:~(#1)}}
	\mdfsetup{
		backgroundcolor=\mdframecolorTheorem,
		linecolor=\mdframecolorTheorem,
		% ----------------------------------
		frametitlerulewidth=\frametitlerulewidththeorem,%    options when using {tcolorbox}?
		roundcorner=\roundcornertheorem,
		linewidth=\linewidththeorem,
		innerbottommargin=\innerbottommargintheorem,
		innerleftmargin=\innerleftmargintheorem,
		innerrightmargin=\innerrightmargintheorem,
		innertopmargin=\innertopmargintheorem,
		outerlinewidth=\outerlinewidththeorem,
		topline=false,
		innertopmargin=-5pt,
		innerbottommargin=1pt,
		linewidth=0,
		startinnercode=\paragraph{{\strut Theorem~\thetheo\theoName}}
	}
	\begin{mdframed}[]\relax%
	}{\end{mdframed}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Corollary
\newenvironment{corollary}[1][]{%
	\refstepcounter{theo}%
\ifstrempty{#1}%
{\newcommand{\theoName}{}}
{\newcommand{\theoName}{:~(#1)}}
\mdfsetup{
	backgroundcolor=\mdframecolorTheorem,
	linecolor=\mdframecolorTheorem,
	% ----------------------------------
	frametitlerulewidth=\frametitlerulewidththeorem,%    options when using {tcolorbox}?
	roundcorner=\roundcornertheorem,
	linewidth=\linewidththeorem,
	innerbottommargin=\innerbottommargintheorem,
	innerleftmargin=\innerleftmargintheorem,
	innerrightmargin=\innerrightmargintheorem,
	innertopmargin=\innertopmargintheorem,
	outerlinewidth=\outerlinewidththeorem,
	topline=false,
	innertopmargin=-5pt,
	innerbottommargin=1pt,
	linewidth=0,
	startinnercode=\paragraph{{\strut Corollary~\thetheo\theoName}}
}
	\begin{mdframed}[]\relax%
	}{\end{mdframed}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Lemma
\newenvironment{lemma}[1][]{%
	\refstepcounter{theo}%
\ifstrempty{#1}%
{\newcommand{\theoName}{}}
{\newcommand{\theoName}{:~(#1)}}
\mdfsetup{
	backgroundcolor=\mdframecolorTheorem,
	linecolor=\mdframecolorTheorem,
	% ----------------------------------
	frametitlerulewidth=\frametitlerulewidththeorem,%    options when using {tcolorbox}?
	roundcorner=\roundcornertheorem,
	linewidth=\linewidththeorem,
	innerbottommargin=\innerbottommargintheorem,
	innerleftmargin=\innerleftmargintheorem,
	innerrightmargin=\innerrightmargintheorem,
	innertopmargin=\innertopmargintheorem,
	outerlinewidth=\outerlinewidththeorem,
	topline=false,
	innertopmargin=-5pt,
	innerbottommargin=1pt,
	linewidth=0,
	startinnercode=\paragraph{{\strut Lemma~\thetheo\theoName}}
}
\begin{mdframed}[]\relax%
}{\end{mdframed}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Proposition
\newenvironment{proposition}[1][]{%
\refstepcounter{theo}%
\ifstrempty{#1}%
{\newcommand{\theoName}{}}
{\newcommand{\theoName}{:~(#1)}}
\mdfsetup{
	backgroundcolor=\mdframecolorTheorem,
	linecolor=\mdframecolorTheorem,
	% ----------------------------------
	frametitlerulewidth=\frametitlerulewidththeorem,%    options when using {tcolorbox}?
	roundcorner=\roundcornertheorem,
	linewidth=\linewidththeorem,
	innerbottommargin=\innerbottommargintheorem,
	innerleftmargin=\innerleftmargintheorem,
	innerrightmargin=\innerrightmargintheorem,
	innertopmargin=\innertopmargintheorem,
	outerlinewidth=\outerlinewidththeorem,
	topline=false,
	innertopmargin=-5pt,
	innerbottommargin=1pt,
	linewidth=0,
	startinnercode=\paragraph{{\strut Proposition~\thetheo\theoName}}
}
\begin{mdframed}[]\relax%
}{\end{mdframed}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%










